Joint Edge-Model Sparse Learning is Provably Efficient for Graph Neural Networks

Due to the significant computational challenge of training large-scale graph neural networks (GNNs), various sparse learning techniques have been exploited to reduce memory and storage costs. Examples include \textit{graph sparsification} that samples a subgraph to reduce the amount of data aggregation and \textit{model sparsification} that prunes the neural network to reduce the number of trainable weights. Despite the empirical successes in reducing the training cost while maintaining the test accuracy, the theoretical generalization analysis of sparse learning for GNNs remains elusive. To the best of our knowledge, this paper provides the first theoretical characterization of joint edge-model sparse learning from the perspective of sample complexity and convergence rate in achieving zero generalization error. It proves analytically that both sampling important nodes and pruning neurons with the lowest-magnitude can reduce the sample complexity and improve convergence without compromising the test accuracy. Although the analysis is centered on two-layer GNNs with structural constraints on data, the insights are applicable to more general setups and justified by both synthetic and practical citation datasets.

==> PF_old.tex <==
\section{Node Classification: Notation, Formulation, and Algorithm}\label{sec: problem_formulation}
% \textbf{feature definition.}  
% We have two discriminative features $\bfp_+, \bfp_- \in \mathbb{R}^d$, and the non-discriminative features are defined as  $\mathcal{P}_s = \{ \bfz \mid \vm{\bfz}{\bfp_+} = \vm{\bfz}{\bfp_-} =0 \}$, which are orthogonal to the discriminative features.
% \textbf{Notations.} We consider the node classification problem given the structured data embedded in an undirected graph $\mathcal{G}(\mathcal{V},\mathcal{E})$, where $\mathcal{V}$ is the set of nodes and $\mathcal{E}$ is the set of edges. 
% For any node $v\in\mathcal{V}$, we use $\bfx_v\in\mathbb{R}^d$ and $y_v\in \{+1, -1\}$ to denote its input feature and corresponding label \footnote{The analysis can be extended to multi-class classification, see Appendix \ref{sec: multi-class}.}. 
% The input $\bfx_v = \bfp + \bfz$ with $\bfp\in \mathcal{P}$. 
% $\mathcal{P}$ are a group of pattern vectors in $\mathbb{R}^d$, and 
% $\bfz \in \mathbb{R}^d$ denotes the disturbance with $\|\bfz\|_{\infty}\le \sigma \|\bfp\|_{2}$. 
% Specifically, $\bfp_+, \bfp_- \in \mathcal{P}$ are the discriminative features, and all the others are non-discriminative (background) features.
% The output $y_v$ belongs to $\{+1, -1\}$ 
% Then, we consider the following data distribution over the graph $\mathcal{G}$.
% The data distribution $(\bfx_v,y_v)$ over graph $\mathcal{G}$ is as follows.
% % Among the patterns in $\mathcal{P}$, some of them are class relevant, which are denoted as the set of discriminative patterns $\mathcal{P}_D$, while the others are irrelevant, which are denoted as the set of non-discriminative patterns $\mathcal{P}_N$. 
% Some of node features are class relevant, while the other nodes contain only class irrelevant patterns. 
% % $\in \mathcal{P}$ as the discriminative features, and all the others are non-discriminative (background) features.
% For any node $v$, its label $y_v$ is determined by the features in the node $v$ and its neighbors.  Namely, the label is positive if the feature vector of node $v$ or any neighbor node of $v$ contains patterns from positive class. 
% For simplification, we do not consider the node which connects to patterns from multiple classes.


 
%We will discuss uniform and non-uniform sampling in the following analysis. 

% \begin{figure}[h]

% \end{figure}

\textbf{Graph neural network model.} 
We consider the node classification problem given the structured data embedded in an undirected graph $\mathcal{G}(\mathcal{V},\mathcal{E})$, where $\mathcal{V}$ is the set of nodes and $\mathcal{E}$ is the set of edges. 
For any node $v\in\mathcal{V}$, we use $\bfx_v\in\mathbb{R}^d$ and $y_v\in \{+1, -1\}$ to denote its input feature and corresponding label\footnote{The analysis can be extended to multi-class classification, see Appendix \ref{sec: multi-class}.}.
The graph neural network considered in this paper contains a hidden layer following by a linear layer, and the hidden layer contains multiple neurons equipped with non-linear aggregator functions.
For any node $v\in\mathcal{V}$, let $\mathcal{N}(v)$ denote the (1-hop) neighbors of 
node $v$ (including itself), 
and we define $\bfX_{\mathcal{N}(v)}\in\mathbb{R}^{d\times |\mathcal{N}(v)|}$ as the collection of the features in $\mathcal{N}(v)$.  Then, we define  the aggregator function  $\text{AGG}$ as
$\text{AGG}(\bfX_{\mathcal{N}(v)},\bfw)$ for a neuron with weights $\bfw$. 
% Following the GraphSAGE in \cite{HYL17}, we consider the max-pooling aggregator function,
% and its mathematical expression is written as
% \vspace{-2mm}
% \begin{equation}\label{eqn:pool_agg}
%     \text{AGG}(\bfX_{\mathcal{N}(v)},\bfw) = \max_{n\in\mathcal{N}(v)}\phi(\vm{\bfw}{\bfx_{n}}).
% \end{equation}
The weights of the neurons in the hidden layer are denoted as $\{\bfw_k \}_{k=1}^{K}$, and the corresponding weights in the fully connected layer are denoted as $\{a_k \}_{k=1}^{K}$. For the convention of notations, we let $\bfW\in \mathbb{R}^{d\times K}$ and $\bfa\in \mathbb{R}^{K}$ be the collections of $\{\bfw_k \}_{k=1}^K$ and $\{a_k \}_{k=1}^K$, respectively,  where $K$ is the number of neurons in the hidden layer.
Therefore, the output of the neural network at node $v$ can be written as:
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{Figure/GNN_2.pdf}
    \caption{Illustration of the graph neural network}
    \label{fig:GNN} 
\end{figure}
\begin{equation}\label{eqn: useless1}
    g(\bfW, \bfa;\bfX_{\mathcal{N}(v)}) = \frac{1}{K}\sum_{k=1}^{K} a_k \cdot\text{AGG}(\bfX_{\mathcal{N}(v)},\bfw_k).
\end{equation}
Note that $c\phi(z) = \text{sign}(c)\phi(|c|z)$ for ReLU function, and only the signs of $\bfa$ play roles in the expressive power of the neural network. Without loss of generality, we randomly initialize $a_k^{(0)}\in\{+1, -1\}$ and only update the value of $\bfW$ during training process. 
% Hence, \eqref{eqn: useless1} can be  re-written as
% \begin{equation}\label{eqn: output1}
%     g(\bfW,\bfU;\bfx) = \frac{1}{K}\sum_{k} \text{AGG}(\bfX_{\mathcal{N}(v)},\bfw_k) - \frac{1}{K} \sum_{k} \text{AGG}(\bfX_{\mathcal{N}(v)},\bfu_k).
% \end{equation}


\textbf{Problem formulation.} 
Given the labels of a subset of the nodes $\mathcal{D}\subseteq \mathcal{V}$, we  
seek a neural network in the form of \eqref{eqn: useless1} such that $ y_v = \text{sign}\big(g(\bfW,\bfa;\bfX_{\mathcal{N}(v)} )\big)$ for any $v$ in $\mathcal{V}$. 
The problem is solved via minimize an empirical risk function (ERF) as
\begin{equation}\label{eqn: ERF}
\begin{split}
    \min_\bfW: \quad \hat{f}_{\mathcal{D}}(\bfW,\bfa^{(0)}) 
    := &-\frac{1}{|\mathcal{D}|}\sum_{ v \in \mathcal{D} } y_v\cdot g\big(\bfW,\bfa^{(0)};\bfX_{\mathcal{N}(v)} \big).
\end{split}
\end{equation} 
To better represent the test (generalization) error, we define the following generalization function:
\begin{equation}\label{eqn: generalization_error}
    I(g(\bfW,\bfa)) = \mathbb{E}_{v\in\mathcal{V}} \max \big\{1 - y_v\cdot g\big(\bfW,\bfa;\bfX_{\mathcal{N}(v)}\big) , 0 \big\}.
\end{equation}
Note that $I(g(\bfW,\bfa)) \ge 0 $, and $I(g(\bfW,\bfa)) = 0 $ only if $y_v\cdot g(\bfW,\bfa;\bfX_{\mathcal{N}(v)})\ge 1$ for all $v\in \mathcal{V}$. 
Then, if $I(g(\bfW,\bfa))=0$, we must have zero test error, where $y_v = \text{sign}(g(\bfW,\bfa;\bfX_{\mathcal{N}(v)}))$.


\subsection{GNN Learning Algorithm via Edge and Model Sparsification}

% \textbf{Stochastic gradient descent.} The neural network training problem is to optimize the following empirical risk function (ERF):
% \begin{equation}\label{eqn: ERF}
% \begin{split}
%     \hat{f}_{\mathcal{D}}(\bfW,\bfa) 
%     = &-\frac{1}{|\mathcal{D}|}\sum_{ v \in \mathcal{D} } y_v\cdot g\big(\bfW,\bfa;\bfX_{\mathcal{N}(v)} \big).
% \end{split}
% \end{equation}
% The optimization is solved using the stochastic gradient descent algorithm with  
% the pseudo-code summarized in Algorithm \ref{Alg}.

\begin{algorithm}[h]
	\caption{Batch gradient descent algorithm}\label{Alg}
	\begin{algorithmic}[1]
		\Require training data $\bfX$, $\{y_v\}_{v\in\mathcal{D}}$,  step size $c_{\eta}$, number of sampled edges $r$, pruning rate $\beta$, and number of iterations $T$;	
		\renewcommand{\algorithmicensure}{\textbf{Divide:}}
		\Ensure the dataset into disjoint subsets $\{\mathcal{D}^{(t)}\}_{t=1}^T$;
		\renewcommand{\algorithmicensure}{\textbf{Initialization:}}
		\Ensure {$\bfW^{(0)}, \bfa^{(0)}$} as
% 		\State \qquad 
		$\bfw_k^{(0)} \sim \mathcal{N}(0, \delta^2\bfI_d)$ and $a_k^{(0)}\sim \text{Uniform}(\{-1, +1\})$ for $k\in[K]$;
		\renewcommand{\algorithmicensure}{\textbf{Pruning:}}
		\Ensure Generate the mask matrix $\bfM$;
% 		\State \textbf{Partition} $\mathcal{D}$ into $T$ disjoint subsets, denoted as $\{\mathcal{D}_t\}_{t=1}^T$;
		\For   {$t'=0, 1, 2, \cdots, T'-1$}
% 		\State \textbf{Sample} $r$ number of neighbors for each node in $\mathcal{V}$;
		\State $\bfW^{(t'+1)}=\bfW^{(t')}-c_{\eta}\cdot \nabla_\bfW \hat{f}^{(t')}_{\mathcal{D}}(\bfW^{(t')},\bfa^{(0)})$;
% 		\State $\bfU^{(t'+1)}=\bfU^{(t')}-c_{\eta}K\nabla \hat{f}^{(t')}_{\mathcal{D}}(\bfW^{(t')},\bfU^{(t')})$;
		\EndFor
		\renewcommand{\algorithmicensure}{\textbf{Set:}}
	    \Ensure $\beta$ rate of neurons with
		lowest magnitude weights in $\bfW^{(T')}$ to $0$ and others to 1, and obtain the corresponding mask $\bfM$;
		\renewcommand{\algorithmicensure}{\textbf{Re-train:}}
		\Ensure
		rewind the weights to the original initialization as $\bfW^{(0)}$;
		\For  {$t=0, 1, 2, \cdots , T$ }
% 		\State \textbf{Sample} $r$ number of neighbors for each node in $\mathcal{V}$;
		\State $\bfW^{(t+1)}=\bfW^{(t)}-c_{\eta}\cdot \nabla_\bfW \hat{f}^{(t)}_{\mathcal{D}^{(t)}}(\bfM \odot \bfW^{(t)}, \bfa^{(0)})$;
% 		\State $\bfU^{(t+1)}=\bfU^{(t)}-c_{\eta}(1-\beta)K\cdot \nabla \hat{f}^{(t)}_{\mathcal{D}^{(t)}}(\bfM_+\odot\bfW^{(t)},\bfM_-\odot\bfU^{(t)})$;
		\EndFor
		\renewcommand{\algorithmicensure}{\textbf{Return:}}
		\Ensure $\bfW^{(T)}$ and $\bfa^{(0)}$.
	\end{algorithmic}
\end{algorithm}


\textbf{Edge sparsification.} Following the GraphSAGE framework \cite{HYL17}, the neighbors of $v$ used at each iteration are sampled as a subset with a fixed size to reduce the computational time, and the aggregation function is implement as max-pooling function
\begin{equation}\label{eqn:pool_agg}
     \text{AGG}(\bfX_{\mathcal{N}_s^{(t)}(v)},\bfw) = \max_{n\in\mathcal{N}^{(t)}_s(v)}\phi(\vm{\bfw}{\bfx_{n}}).
\end{equation}
% The sampled subset with respect to node $v$ is denoted as $\mathcal{N}_s(v)$ with $|\mathcal{N}_s(v)| =r$. 
% That is, $\mathcal{N}_s(v)$ is a subset of $\mathcal{N}(v)$ with size of $r$.
where $\mathcal{N}_s^{(t)}(v)$ denotes the sampled subset of neighbors of node $v$ at iteration $t$. 
Then, the gradient calculated at iteration $t$ is 
\begin{equation}\label{eqn: ERF_t}
    \begin{split}
        \nabla\hat{f}_{\mathcal{D}}^{(t)}(\bfW,\bfa^{(0)}) 
        = &-\frac{1}{|\mathcal{D}|}\sum_{ v \in \mathcal{D}} y_v\cdot \nabla_\bfW g\big(\bfW, \bfa^{(0)};\bfX_{\mathcal{N}_s^{(t)}(v)} \big).
\end{split}
\end{equation}
\begin{figure}[h]
    \begin{minipage}{0.50\linewidth}
        \centering
    \includegraphics[width=0.7\linewidth]{Figure/sampling.pdf}
    \caption{Illustration of the edge sparsification: a subset of the (1-hop) neighbors in the aggregation}
    \label{fig:sampling_1}
    \end{minipage}
    ~
    \hfill
    \begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=0.95\linewidth]{Figure/IHT.pdf}
    \caption{Illustration of the model sparsification: dash line denote the removed neurons and corresponding weights}
    \label{fig:sampling_2}
    \end{minipage}
    \vspace{-4mm}
\end{figure}

\textbf{Model sparsification.} Similar to \cite{CSCZW21}, we introduce the mask matrix $\bfM\in\{ 0 , 1 \}^{d\times K}$. After the algorithm convergences via training on the original graph neural network, we remove $\beta$ rate of the neurons with lowest-magnitude weights from the model, and the mask matrix $\bfM$ is updated by setting the pruning neurons' columns into $\bfzero$. Then, we rewind the GNN's weights into the original initialization $\bfW^{(0)}, \bfa^{(0)}$, and the data are re-trained on the model $\bfM\odot \bfW$, where $\odot$ stands for entry-wise multiplication.   
% \begin{algorithm}[h]
% 	\caption{Magnitude pruning for model weights}\label{Alg2}
% 	\begin{algorithmic}[1]
% 		\State \textbf{Input:} training data $\bfX$, $\{y_v\}_{v\in\mathcal{D}}$, gradient step size $\eta$, and pruning rate $p$;
% 		\State \textbf{Initialization:} {$\bfW^{(0)}, \bfU^{(0)}$} as
% % 		\State \qquad 
% 		$\bfw_k^{(0)}, \bfu_k^{(0)} \sim \mathcal{N}(0, \delta^2\bfI_d)$ for $k\in[K]$;
% % 		\State \textbf{Pruning:} Generate the mask matrix $\bfM_+$ and $\bfM_-$ using Algorithm \ref{alg2}
% % 		\State \textbf{Partition} $\mathcal{D}$ into $T$ disjoint subsets, denoted as $\{\mathcal{D}_t\}_{t=1}^T$;
% 		\For  {$t=0, 1, 2, \cdots, T'-1$}
% % 		\State \textbf{Sample} $r$ number of neighbors for each node in $\mathcal{V}$;
% 		\State $\bfW^{(t+1)}=\bfW^{(t)}-\eta\nabla \hat{f}^{(t)}_{\mathcal{D}}(\bfW^{(t)},\bfU^{(t)})$;
% 		\State $\bfV^{(t+1)}=\bfV^{(t)}-\eta\nabla \hat{f}^{(t)}_{\mathcal{D}}(\bfW^{(t)},\bfU^{(t)})$;
% 		\EndFor
% 		\State \textbf{Set} rate $p_M$ of the
% 		lowest magnitude neurons in $\bfW^{(T')}$ and $\bfU^{(T')}$ to $0$ and others to 1, and obtain the corresponding mask $\bfM_+$ and $\bfM_-$;\\
% 		\Return $\bfM_+$ and $\bfM_-$.
% 	\end{algorithmic}
% \end{algorithm}


\iffalse
\begin{algorithm}[h]
	\caption{Stochastic gradient descent algorithm}\label{Alg}
	\begin{algorithmic}[1]
		\State \textbf{Input:} training data $\bfX$, $\{y_v\}_{v\in\mathcal{D}}$, and gradient step size $\eta$;
		\State \textbf{Initialization:} {$\bfW^{(0)}, \bfU^{(0)}$} as
% 		\State \qquad 
		$\bfw_k^{(0)}, \bfu_k^{(0)} \sim \mathcal{N}(0, \delta^2\bfI_d)$ for $k\in[K]$;
% 		\State \textbf{Partition} $\mathcal{D}$ into $T$ disjoint subsets, denoted as $\{\mathcal{D}_t\}_{t=1}^T$;
		\For  {$t=0, 1, 2, \cdots, T-1$}
		\State \textbf{Sample} $r$ number of neighbors for each node in $\mathcal{V}$;
		\State $\bfW^{(t+1)}=\bfW^{(t)}-\eta\nabla \hat{f}_{\mathcal{D}}^{(t)}(\bfW^{(t)},\bfU^{(t)})$;
		\State $\bfV^{(t+1)}=\bfV^{(t)}-\eta\nabla \hat{f}_{\mathcal{D}}^{(t)}(\bfW^{(t)},\bfU^{(t)})$;
		\EndFor\\
		\Return $\bfW^{(T)}$ and $\bfU^{(T)}$.
	\end{algorithmic}
\end{algorithm}
\fi

==> Theorem.tex <==
\section{Theoretical Analysis}\label{sec: theoretical_results}
% For the convenience of presentation, we define $\alpha$ as the sampling rate of important edges that connects the nodes with discriminative patterns.
% A sampling strategy with $\alpha$ greater than $r/M$ can be viewed as importance sampling when sampling $r$ out of $M$ neighbors nodes.
% Also, we denote $\beta$ as the pruning rate of neurons such that $\beta = 1 - \frac{\|\bfM_+\|_0+\|\bfM_-\|_0}{2Kd}$.
% The computational complexity per iteration is in the order of the number of sampled nodes $r$ and model size $(1-\beta)K$, we refer the computation complexity as $T\times r\times (1-\beta)K$ in the following discussion.

\subsection{Takeaways of the Theoretical Findings}
Our theoretical analysis is built upon the data distribution $(\bfx_v,y_v)$ over graph $\mathcal{G}$ as follows.
% Among the patterns in $\mathcal{P}$, some of them are class relevant, which are denoted as the set of discriminative patterns $\mathcal{P}_D$, while the others are irrelevant, which are denoted as the set of non-discriminative patterns $\mathcal{P}_N$. 
Some of node features are class relevant, while the other nodes contain only class irrelevant patterns. 
% $\in \mathcal{P}$ as the discriminative features, and all the others are non-discriminative (background) features.
For any node $v$, its label $y_v$ is determined by the features in the node $v$ and its neighbors.  For instance, the label is positive if the feature vector of node $v$ or any neighbor node of $v$ contains patterns from positive class. 
For simplification, we do not consider the node which connects to patterns from multiple classes. Before formally presenting them, we summarize the highlights as follows.

\textbf{(T1) Sample complexity and convergence analysis for guaranteed zero generalization error.}
The learned model achieves zero generalization with finite number of training samples and computational time, which are the polynomial functions of some graph topology parameters and the inverse of model complexity $K^{-1}$.


\textbf{(T2) The influence of the graph typology.}
The required number of samples depends on the degree of the graph and sampling rate of important edges, which are affected by the edge sparsification algorithms.
By sampling $r$ out of $M$ neighbor nodes for the training data, the sample complexity is reduced to $1+r^2$ from $1+M^2$. 
Nevertheless, the sampling rate of important edges is reduced accordingly in general, and the algorithm requires more training samples and larger iterations for convergence.
With random sampling, the sample complexity and computational complexity are irrelevant with $r$, which indicates no improvement with sampling. 
However, with importance sampling algorithms such that the sampling rate of important edges are higher than the random sampling rate, both the sample complexity and the computational time can be both improved.

\textbf{(T3) The influence of the model complexity.}
With a larger number of neurons, the sample complexity is reduced as a function of $1/K$. 
This result not only provides the verification of the wide-usage of overparameterized model but also indicates the non-triviality of model sparsification, where random model pruning will only lead to performance degradation.
Our theorem shows that
the neuron weights with large magnitudes tend to be concentrated in the direction of discriminative patterns, which might be a possible explanation for the widely-used magnitude-based model pruning method. 
Therefore, removing neurons with small magnitudes can prevent  the model from learning the class irrelevant patterns, by which the model is less likely to be overfitting. Specifically, the algorithm can tolerant higher noise in the input features, and the training on the pruned model achieves a faster convergence with smaller sample complexity.

\textbf{(T4) Edge sparsification and model sparsification are win-win in efficient learning.}
Our theorem provides a theoretical validation for the joint edge-model sparsification. 
Edge sparsification improves the learning efficiency via removing random class irrelevant patterns in input and reducing the dependence among training data. As for model sparsification, neurons with bad initialization are discarded, and the remaining neurons are tended to learn class relevant patterns compared with training on the original dense network. These two sparsification techniques are not mutually  exclusive and can be applied together. 
 

% \textbf{(A) Importance neighbor sampling of graph structured data can save the sample complexity and computational time.}
% Both the required training sample amount and number of iterations for convergence reduce when the sampling rate of important edges increases or the number of sampled neighbor nodes decreases. With random sampling such that $\alpha = r/M$, the sample complexity and computational complexity are irrelevant with $r$, which indicates no improvement with sampling. Nevertheless, when the importance sampling is implemented, where $\alpha$ is improved by a constant or in the order of $r$ compared with random sampling, the sample complexity and the computational time can be both improved.  
% % With the increase of sampling rate of the important edges that are connected with nodes with discriminative patterns, we have both reduced training samples and small number of iterations for the convergence. 

% \textbf{(B) Magnitude-based neuron pruning in GNNs leads to fast convergence rate and improved generalization.}
% Our theorem shows that
% the neuron weights with large magnitudes tend to be concentrated in the direction of discriminative patterns. 
% Therefore, removing neurons with small magnitudes can reduce the model ability in learning the non-discriminative patterns, by which the model is less likely to be overfitting. Specifically, the algorithm can tolerant higher noise, and the learned model achieves a faster convergence and better generalization. 
% % Suppose the rate of lucky neurons is improved to $\beta$ after pruning, the number of iterations and sample complexity are improved in the speed of $1/\beta$ and $1/\beta^2$, respectively. 

% \textbf{(C) Overparameterization improves the generalization.} With larger neurons, the algorithm requires fewer samples for convergence and enjoys a faster convergence rate. This result not only provide the verification of the wide-usage of overparameterized model but also indicates the non-triviality of graph and model sparsification, where random pruning on graph or model will only lead to performance degradation.

% \subsection{Assumptions, Technique Challenges, and Novelties.} 
\subsection{Formal Theoretical Results}\label{sec: formal_theoretical}
\textbf{Assumptions and notations.} 
% The data distribution $(\bfx_v,y_v)$ over graph $\mathcal{G}$ is as follows.
% % Among the patterns in $\mathcal{P}$, some of them are class relevant, which are denoted as the set of discriminative patterns $\mathcal{P}_D$, while the others are irrelevant, which are denoted as the set of non-discriminative patterns $\mathcal{P}_N$. 
% Some of node features are class relevant, while the other nodes contain only class irrelevant patterns. 
% % $\in \mathcal{P}$ as the discriminative features, and all the others are non-discriminative (background) features.
% For any node $v$, its label $y_v$ is determined by the features in the node $v$ and its neighbors.  Namely, the label is positive if the feature vector of node $v$ or any neighbor node of $v$ contains patterns from positive class. 
% For simplification, we do not consider the node which connects to patterns from multiple classes.
The input feature is modeled as $\bfx_v = \bfp_v + \bfz_v$ with $\bfp_v\in \mathcal{P}$ for $v\in\mathcal{V}$, where  
$\mathcal{P}$ is a group of normalized pattern vectors in $\mathbb{R}^d$, and 
$\bfz_v \in \mathbb{R}^d$ denotes the disturbance with $\|\bfz\|_{2}\le \sigma$. Also, we use $\mathcal{P}_+$, $\mathcal{P}_-$ to denote the discriminative patterns that relevant to the positive and negative labels, and $\mathcal{P}_{{N}}$ indicates the set of class irrelevant patterns. With these notations,  
we consider a general distribution with assumptions below: (\textbf{A1}) the patterns in $\mathcal{P}$ are orthogonal to each other;
(\textbf{A2}) the discriminative patterns of different classes are identically distributed in the graph structured data,  and the class probabilities are balanced, namely $\text{Prob}(y = +1) = \text{Prob}(y = -1) = 1/2$;
(\textbf{A3}) any non-discriminative pattern is distributed independently with other patterns and uniformly in nodes of all classes.
To make the analysis feasible, we consider the case of one discriminative pattern for each class. Namely, $\mathcal{P}_+ = \bfp_+$ and $\mathcal{P}_- = \bfp_-$. While $\mathcal{P}_N$ can contain arbitrarily large number of patterns as long as they are orthogonal. 
Hence, we have $\text{Prob}(\bfp_+) = \text{Prob}(\bfp_-)$ and $\text{Prob}({\bfp | y= +1}) = \text{Prob}({\bfp | y= -1})$ for any $\bfp\in\mathcal{P}_N$.
% Then, (\textbf{A2}) is equivalent to that the distributions of $\bfp_+$ and $\bfp_-$ are identical in the graph structured data.

We use $h_1(t) = \Omega\big(h_2(t)\big) (\text{or }~\mathcal{O}\big(g(t)\big))$ to denote $h_1(n)\ge (\text{or } \le)~C\cdot h_2(t)$ for some large constant $C$ and sufficiently large $t$.
Moreover,
$L:=|\mathcal{P}|$ denotes the elements in $\mathcal{P}$, $r:=|\mathcal{N}_s(v)|$ denotes the number of nodes sampled for each node during each iteration. Next, we define $\alpha$ as the sampling rate of important edges that connects the nodes with discriminative patterns.
A sampling strategy with $\alpha$ greater than $r/M$ can be viewed as importance sampling when sampling $r$ out of $M$ neighbors nodes.
Also, we denote $\beta$ as the pruning rate of neurons such that $\beta = 1 - \frac{\|\bfM\|_0}{Kd}$. The computation complexity is calculated as the multiplication of the size of pruned model, the size of aggregated neighbor nodes, and number of iterations.  
% The computational complexity per iteration is in the order of the number of sampled nodes $r$ and model size $(1-\beta)K$, we refer the computation complexity as $T\times r\times (1-\beta)K$ in the following discussion.

% A detailed proof sketchy can be found in Appendix \ref{sec: max-pooling}.


% \begin{theorem}[Mean-pooling aggregator]\label{Thm:major_thm2}
% Suppose the number of training samples satisfies
% \begin{equation}
%     N = \Omega\big(\textcolor{red}{(1-3\varepsilon)^{-2}\alpha^{-2}}(1+r^2)r^2 M^2 d\log q\big).
% \end{equation}
% Then,
% after $T$ number of iterations such that
% \begin{equation}
%     T \ge \Omega\Big( \frac{M^2}{(1-3\varepsilon) \alpha K} \Big),
% \end{equation}
% the generalization function in \eqref{eqn: generalization_error} satisfies
% \begin{equation}
%     I\big(g(\bfW^{(T)},\bfU^{(T)})\big) = 0.
% \end{equation}
% \end{theorem}

% \textbf{Convergence to a good GNN.}
% Theorem \ref{Thm:major_thm} characterizes the performance of Algorithm \ref{Alg} in learning graph structured data via graph sparsification. On the one hand, by sampling $r$ out of the neighbor nodes for each training data, the sample complexity is reduced to the order of $1+r^2$. In addition, both the sample complexity and convergence rate are improved when sampling rate of the edges that connects discriminative features increase. On the other hand, by applying magnitude pruning methods on the neuron weights, we observe improved sample complexity and reduced number of iterations to achieve zero generalization. 

Theorem \ref{Thm:major_thm} characterizes the performance of Algorithm \ref{Alg} in learning graph structured data via graph sparsification.
The returned model achieves zero generalization error from \eqref{eqn: zero_generalization} if (\textbf{C1}) the number of training samples exceeds the bound in \eqref{eqn: number_of_samples}; 
%  Second, the neurons in the hidden layer is sufficiently large as shown in \eqref{eqn: number_of_neurons}. 
(\textbf{C2}) the algorithm requires at least $T$  iteration  in \eqref{eqn: number_of_iteration} for convergence. The total computation complexity is in the order of \eqref{eqn: cc} if we ignore the pruning stage.
\begin{theorem}\label{Thm:major_thm}
Given the bounded noise such that $\sigma < {1}/{L}$ and sufficient complex model such that $K>L^2\cdot\log q$ for some constant $q>0$. 
Suppose the following conditions hold:
\begin{enumerate}
    \item the number of training samples satisfies 
\begin{equation}\label{eqn: number_of_samples}
    |\mathcal{D}| = \Omega\big({ (1+L^2\sigma^2+K^{-1})\cdot \alpha^{-2}}\cdot (1+r^2)\cdot  (1-\beta)^2 \cdot  L^2\cdot \log q\big);
\end{equation}
%     \item the number of neurons satisfies
% \begin{equation}\label{eqn: number_of_neurons}
%     K = \Omega\big( L^2\cdot \log q \big);
% \end{equation}
    \item 
    after $T$ number of iterations such that
    \begin{equation}
    \label{eqn: number_of_iteration}
        T = \Omega\big((1+N^{-1/2})\cdot(1+L\sigma+K^{-1/2}) \cdot (1-\beta)\cdot\alpha^{-1} \cdot L \big).
    \end{equation}
\end{enumerate}
Then, with probability at least $1-q^{-10}$, the model returned by Algorithm \ref{Alg} achieves zero generalization error as
\begin{equation}\label{eqn: zero_generalization}
    I\big(g(\bfW^{(T)},\bfU^{(T)})\big) = 0.
\end{equation}
In addition, the computational complexity for achieving zero generalization error is 
\begin{equation}\label{eqn: cc}
    % \text{Time} 
    h= \mathcal{O}\big((1-\beta)Kd\cdot r\cdot T\cdot |\mathcal{D}|\big) = \mathcal{O}\big((1-\beta)^2\alpha^{-1}r\cdot KdL\cdot |\mathcal{D}|\big).
\end{equation}
\end{theorem}

 
 
%  From Theorem \ref{Thm:major_thm}, the factor $\varepsilon$ is a linear function of $1/\sqrt{K}$ with a negative slope, where $K$ is the number of neurons. More neurons indicates a smaller $\varepsilon$, and both the sample complexity in \eqref{eqn: number_of_samples} and convergence rate in \eqref{eqn: number_of_iteration} are improved.
% Suppose the degree of the graph is $M$, random sampling strategy indicates that the sampling rate of important edges $\alpha$ is $r/M$. As the number of samples and computation complexity are both constant, which shows no improvement or degradation in computational complexity. Instead, applying any importance sampling such that $\alpha$ is larger than $r/M$, the learning performance can be improved in both sample complexity and convergence rate.
% When the pruning rate $\beta$ increases, the sample complexity in \eqref{eqn: number_of_samples}  and the number of iterations in \eqref{eqn: number_of_iteration} reduce, which indicates an improved learning performance. Specifically, the number of iterations is reduced as a linear function of $\beta$, while the other two are reduced as a quadratic function of $1-\beta$.

\textbf{Technique novelty and challenges.} 
The techniques used in this paper are mainly inspired by the feature learning framework in analyzing convolution neural networks \citep{SWL22,BG21}. 
Most importantly, we generalize the analysis to handle the graph sparsification techniques, and the major challenges include addressing the mismatch of the input features and labels due to sub-sampling and the characterization of magnitude and angle of the convergence neuron weights.
Next, different from CNN model, the labels of graph structured data are partly dependent even if the feature vectors are assumed to be independent.
Moreover, as the labels are distinguished by the feature vectors, the patterns need to be separable for different classes. In this paper, we relax the standard assumption of the orthogonality among the patterns \citep{SWL22,BG21} by adding a disturbance vector $\bfz$ in the input feature.
Last, compared with the NTK framework \citep{ALL19,JGH18},  this paper considers a less overparameterized model such that $K=\Omega(L^2)$\footnote{Take \citep{ALL19} for example, $K$ should be at least in the order of $\text{poly}(M,L)$ because the $p$ in \citep{ALL19} is at least $ML$ for our data distribution.}, where one cannot use a linear network to approximate the original network. The problems are highly non-convex, and the VC-dimension of the model over the data distribution is at least an exponential function of the dimension (see Appendix \ref{app: VC} for the full proof).    

 
